Reachability-based Trajectory Design with Neural Implicit Safety Constraints

Generating safe motion plans in real-time is a key requirement for deploying robot manipulators to assist humans in collaborative settings. In particular, robots must satisfy strict safety requirements to avoid self-damage or harming nearby humans. Satisfying these requirements is particularly challenging if the robot must also operate in real-time to adjust to changes in its environment.This paper addresses these challenges by proposing Reachability-based Signed Distance Functions (RDFs) as a neural implicit representation for robot safety. RDF, which can be constructed using supervised learning in a tractable fashion, accurately predicts the distance between the swept volume of a robot arm and an obstacle. RDF's inference and gradient computations are fast and scale linearly with the dimension of the system; these features enable its use within a novel real-time trajectory planning framework as a continuous-time collision-avoidance constraint. The planning method using RDF is compared to a variety of state-of-the-art techniques and is demonstrated to successfully solve challenging motion planning tasks for high-dimensional systems faster and more reliably than all tested methods.

==> algorithms/pzfk.tex <==
%          %~~~~~~~~~~~~ Compose FK
% \begin{algorithm}[t]
% \small
% \jon{define pzHomTrans}
% \begin{algorithmic}[1]

% \State{\bf parfor} $i = 1:\nt$ %// parallel for each time step

% \State\hspace{0.2in}{\bf for} $j = 1:\nq$ %// for each joint
%     \State\hspace{0.4in}$\pz{p_j}(\pzqi) \leftarrow \pz{\mathbf{0}}$ %// initialize frame location 
        
%     \State\hspace{0.4in}$ \pz{R_j}(\pzqi) \leftarrow \pz{I_{3 \times 3}}$ %// initialize frame orientation
    
%      \State\hspace{0.4in}{\bf for} $l = 1:j$

%         \State\hspace{0.6in}$\pz{R_{l}^{l-1}}(\pzqli), \pz{\nom{p\lssmu}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
%         \State\hspace{0.6in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi)  \odot \pz{p_{l}^{l-1}}$
        
%         \State\hspace{0.6in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_j}(\pzqi) \odot  \pz{R_{l}^{l-1}}(\pzqli)$ 

%     \State\hspace{0.4in}{\bf end for}
    
%     \State\hspace{0.4in}$\pz{\FK_j}(\pzqi) \leftarrow \{ \pz{R_j}(\pzqi) ,  \pz{p_j}(\pzqi) \}$ 
  
    
% \State\hspace{0.2in}{\bf end for}

% \State{\bf end parfor}

% \end{algorithmic}
% \caption{\small $\{\pz{\FK_j}(\pzqi)\,:\, j \in \Nq,\ i \in \Nt \} = \texttt{PZFK}(\{ \pzi{q_j} \,:\, j \in \Nq,\ i \in \Nt \})$}
% \label{alg:compose_fk}
% \end{algorithm}


%~~~~~~~~~~~~ Compose FK
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

% \State{\bf parfor} $i = 1:\nt$ %// parallel for each time step
\State $\pz{p_0}_i(\pzqji) \leftarrow \pz{\mathbf{0}}$
\State $\pz{R_0}_i(\pzqji) \leftarrow \pz{I_{3 \times 3}}$

\State\hspace{0in}{\bf for} $j = 1:\nq$ %// for each joint

    % \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{\nom{p\jssmu}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
    \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{\nom{p\jssmu}} \leftarrow \pz{\homtrans_{j}^{j-1}}(\pzqji)$ as in \eqref{eq:homogeneous_transform}
    
    \State\hspace{0.2in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_{j-1}}(\pzqi) \oplus \pz{R_{j-1}}(\pzqi) \pz{p_{j}^{j-1}}$
        
    \State\hspace{0.2in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_{j-1}}(\pzqi)  \pz{R_{j}^{j-1}}(\pzqji)$ 
    
    \State\hspace{0.2in}$\pz{\FK_j}(\pzqi) \leftarrow \{ \pz{R_j}(\pzqi) ,  \pz{p_j}(\pzqi) \}$ 
    
\State\hspace{0in}{\bf end for}
\State \textbf{Return} $\{\pz{\FK_j}(\pzqi)\,:\, j \in \Nq \}$

% \State{\bf end parfor}

\end{algorithmic}
\caption{\small $ \texttt{PZFK}(\pzqi)$}
\label{alg:compose_fk}
\end{algorithm}

==> algorithms/pzfo.tex <==
         %~~~~~~~~~~~~ Compose FK
% \begin{algorithm}[t]
% \small
%  \jon{define pzHomTrans}
% \begin{algorithmic}[1]


% \State{\bf parfor} $i = 1:\nt$ %// parallel for each time step

% \State\hspace{0.2in}{\bf for} $j = 1:\nq$ %// for each joint
%     \State\hspace{0.4in}$\pz{p_j}(\pzqi) \leftarrow \pz{\mathbf{0}}$ %// initialize frame location 
        
%     \State\hspace{0.4in}$ \pz{R_j}(\pzqi) \leftarrow \pz{I_{3 \times 3}}$ %// initialize frame orientation
    
%      \State\hspace{0.4in}{\bf for} $l = 1:j$

%         \State\hspace{0.6in}$\pz{R_{l}^{l-1}}(\pzqli), \pz{\nom{p\lssmu}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
%         \State\hspace{0.6in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi)  \odot \pz{p_{l}^{l-1}}$
        
%         \State\hspace{0.6in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_j}(\pzqi) \odot  \pz{R_{l}^{l-1}}(\pzqli)$ 

%     \State\hspace{0.4in}{\bf end for}
    

%      \State\hspace{0.4in}$\pz{\FO_j}(\pzqi) \leftarrow \pz{p_j}(\pzqi) \oplus  \pz{R_j}(\pzqi) \odot \pz{L_j}$ 
  
    
% \State\hspace{0.2in}{\bf end for}

% \State{\bf end parfor}

% \end{algorithmic}
% \caption{\small $\{\pz{\FO_j}(\pzqi)\,:\, j \in \Nq,\ i \in \Nt \} = \texttt{PZFO}(\{ \pzi{q_j} \,:\, j \in \Nq,\ i \in \Nt \})$}
% \label{alg:compose_fo}
% \end{algorithm}


\begin{algorithm}[t]
\begin{algorithmic}[1]
\State $\{\pz{\FK_j}(\pzqi)\,:\, j \in \Nq \} \leftarrow \texttt{PZFK}(\pzqi)$
\State{\bf for} $j = 1:\nq$ %// for each joint
     \State\hspace{0.2in}$\pz{\FO_j}(\pzqi) \leftarrow \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi) \pz{L_j}$ 
\State{\bf end for}
\State \textbf{Return}$\{\pz{\FO_j}(\pzqi)\,:\, j \in \Nq\}$
\end{algorithmic}
\caption{$\texttt{PZFO}(\pzqi, \{\pz{L_j} \,:\,\ j \in \Nq\})$}
\label{alg:compose_fo}
\end{algorithm}

==> algorithms/slice.tex <==
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
    \State // Let $Z = (x,g^i,\sym{\beta^i})^p$ denote the input zonotope or rotatotope

    \State  $Z_{\regtext{sliced}} \leftarrow (x,g^i,\sym{\beta^i})^p$ // allocate output

    \State{\bf for} $i = 1,\cdots,p$ // iterate over generator/indeterminate pairs
    
    \State\hspace{0.2in}{\bf for} $j = 1,\cdots,n$  // iterate over input values
    
    \State\hspace{0.4in}{\bf if} $\sym{\sigma^j} \in \sym{\beta^i}$
    
    \State\hspace{0.6in} $g^i \leftarrow \sigma^j g^i$ // multiply generator by value
    
    \State\hspace{0.6in} $\sym{\beta^i} \leftarrow \sym{\beta^i} \setminus \sym{\sigma^j}$ // remove evaluated indeterminate

    \State\hspace{0.4in}{\bf end if}
    
    \State\hspace{0.2in}{\bf end for}
    
    \State\hspace{0.2in}{\bf if} $\sym{\beta^i} = \emptyset$ // if fully-sliced, then $g^i$ is no longer needed
    
    \State\hspace{0.4in} $x \leftarrow x + g^i$ and $g^i \leftarrow \emptyset$ // shift center, remove generator
    
    % \State\hspace{0.4in} $g^i \leftarrow \emptyset$ // generator is no longer needed 
    
    \State\hspace{0.2in}{\bf end if}
    
    \State{\bf end for}
    
    \end{algorithmic}
\caption{\small $Z_{\regtext{sliced}} = \slice\left(Z, \{\sym{\sigma^j}\}_{j=1}^n, \{\sigma^j\}_{j=1}^n\right)$}
\label{alg:slice}
\end{algorithm}

==> sections/reachability.tex <==
\section{Reachability Analysis}\label{sec:reachability}


\begin{itemize}
    \item 

    In particular, we describe how we use zonotopes to overapproximate the forward occupancy of the robot and obstacles, and then use those approximations to overapproximate their distance. 

    \item We make the following assumptions:
    \begin{assum}
    We overapproximate each link of the robot using the smallest enclosing bounding box.
    All obstacles are cuboids of the same size.
    We assume that reachable sets of the robot and the cuboids representing the obstacles can be overapproximated using polytopic set-based representations.
    \end{assum}
\end{itemize}


\subsection{Polynomial Zonotope Trajectory Representation}
\label{subsec:pz_traj_rep}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.97\textwidth]{figures/rdf_reachability.pdf}
    \caption{Visualization of polynomial zonotope representations of the entire FRS and the subset corresponding to a single trajectory.}
    \label{fig:example_polyzono}
\end{figure*}

This subsection describes how \methodname applies polynomial zonotope arithmetic to overapproximates the robot's parameterized desired trajectories, as in Def. \ref{def:traj_param}, to conservatively account for continuous time our optimization framework.
Our approach to overapproximate trajectories of the robot.
Recall that as a result of Def. \ref{defn:traj_param}, the initial condition of the desired trajectories at each planning iteration is known.
% before any optimization problem needs to be solved.
As a result, the desired trajectories $\qdesk$ are functions of only time $t$ and the trajectory parameter $k$.
Our approach begins by creating polynomial zonotope versions of $T$ and $K$, which are then plugged into the formula for $\qdesk$ to create polynomial zonotopes representing the desired trajectories.

\subsubsection{Time Horizon PZs}
We first describe how to create polynomial zonotopes representing the planning time horizon $T$.
We choose a timestep $\timestep$ so that $\nt \coloneqq \frac{T}{\timestep} \in \N$.
Let $N_t := \{1,\ldots,\nt\}$.
Divide the compact time horizon $T \subset \R$ into $\nt$ time subintervals.
% For example, if $T = [0, 1]$ and $\timestep = 0.01$, then the time horizon is divided into $\nt = 100$ subintervals.
Consider the $i$\ts{th} time subinterval corresponding to $t \in \iv{(i-1)\timestep, i\timestep}$.
We represent this subinterval as a polynomial zonotope $\pz{T_i}$, where 
\begin{equation}
    \label{eq:time_pz}
    \pz{T_i} =
        \left\{t \in T \mid 
            t = \tfrac{(i-1) + i}{2}\timestep + \tfrac{1}{2} \timestep \tvari,\ \tvari \in [-1,1]
        \right\}
\end{equation}
with indeterminate $\tvari \in \iv{-1, 1}$.

\subsubsection{Trajectory Parameter PZs}
\label{subsubsec: pz_traf}
Now we describe how to create polynomial zonotopes representing the set of trajectory parameters $K$.
In this work, we choose $K = \bigtimes_{i=1}^{n_q} K_i$, where each $\Kj$ is the compact one-dimensional interval  $\Kj = \iv{-1, 1}$.
We represent the interval $\Kj$ as a polynomial zonotope $\pz{\Kj} = \kjvar$ where $\kjvar \in \iv{-1, 1}$ is an indeterminate.
We let $\kvar \in \iv{-1,1}^{n_q}$ denote the vector of indeterminates where the $j$\ts{th} component of $\kvar$ is $\kjvar$.
With this choice of $\Kj$, any particular $k_j$ directly yields $k_j = \setop{slice}(\pz{\Kj}, \kjvar, k_j)$ (see \eqref{eq:pz_slice}).
In other words, plugging in $k_j$ to the indeterminate $\kjvar$ yields the subset of $\pz{\Kj}$ which is $k_j$ itself.
In fact, the process of ``slicing'' a polynomial zonotope by a trajectory parameter is critical to our formulation of the constraints within \methodname.

\subsubsection{Desired Trajectory PZs}
The desired position, velocity, and acceleration trajectories of the robot, defined in Def. \ref{def:traj_param}, are functions of both time $t$ and the trajectory parameter $k$.
Using the time partition and trajectory parameter polynomial zonotopes described above, we create polynomial zonotopes $\pzqdesji$ that overapproximate $\qdeskj$ for all $t$ in the $i$\ts{th} time subinterval and $k \in K$ by plugging the polynomial zonotopes $\pz{T_i}$ and $\pz{K}$ into the formula for $\qdeskj$.

\begin{lem}[Desired Trajectory PZs]
\label{lem:pz_desired_trajectory}
The desired trajectory polynomial zonotopes $\pzqdesji$ are overapproximative, i.e., for each $j \in \Nq$, $\pzqdesji$ satisfies
\begin{equation}
    \qdeskj \in \pzqdesji \quad \forall t \in \pz{T_i}, \, k \in \pz{K}.
\end{equation}
One can similarly define $\pzqddesji$, and $\pzqdddesji$ that are also overapproximative.
\end{lem}
\begin{proof}
\jon{See ARMOUR}The desired trajectory $\qdeskj$ is an analytic function that depends only on time $t$ and $k$, which are included in $\pz{T_i}$ and $\pz{K}$.
All operations involving polynomial zonotopes are either exact or overapproximative for analytic functions \cite[Section 2.D]{kochdumper2020sparse}, so $\pz{T_i}$ and $\pz{K}$ in place of the arguments $t$ and $k$ yields an overapproximative polynomial zonotope.
\end{proof}

\subsubsection{Slicing Yields Desired Trajectories}
Recall that $\pz{T_i}$ and $\pz{K_j}$ have indeterminates $\tvari$ and $\kjvar$ respectively.
Because the desired trajectories only depend on $t$ and $k$, the polynomial zonotopes $\pzqdesji$, $\pzqddesji$ and $\pzqdddesji$ depend only on the indeterminates $\tvari$ and $\kvar$.
By plugging in a given $k$ for $\kvar$ via the $\setop{slice}$ operation, we obtain a polynomial zonotope where $\tvari$ is the only remaining indeterminate. 
Because we perform this particular slicing operation repeatedly throughout this document, if we are given a polynomial zonotope, $\pzqdesji$, we use the shorthand $\pzqdesjki = \setop{slice}(\pzqdesji, \kvar, k)$.
Notice that because of our previous observation, $\qdeskj \in \pzqdesjki$ for all $t \in \pz{T_i}$ (and similarly for $\pzqddesjki$ and $\pzqdddesjki$).


\subsection{Reachable Set Construction}
We first generate polynomial zonotopes for the overapproximation of cosine and sine of joint trajectory with a given initial state as $(\pz{\cos{q(T;K)}}, \pz{\sin{q(T;K)}})$ \cite{holmes2020armtd}. In short, let's notate $\pz{\text{c}_q(T;K)}=\pz{\cos{q(T;K)}}$ and $\pz{\text{s}_q(T;K)}=\pz{\sin{q(T;K)}}$. Then, we can construct matrix polynomial zonotope to represent overapproximated rotational operation of each joint trajectory as follow.

After generating the polynomial zonotope overapproximations of joint trajectories in the previous subsection, \methodname composes these together to bound the kinematic behavior of the arm and the possible torques required to achieve these trajectories.
We formulate algorithms which generate polynomial zonotopes (parameterized by $k$) describing the volume occupied by the arm and the motor torques required to track a given trajectory.
These algorithms run at the beginning of each planning iteration, and their outputs are used to formulate constraints on $k$ which overapproximate those in \eqref{eq:optpos} - \eqref{eq:optcolcon}. \jon{fix this}
In the remainder of this subsection, we describe how to compute reachable sets for a single joint/link over a single interval of time.

\subsubsection{Forward Kinematics Reachable Set}
We reformulate the robot's forward kinematics \eqref{eq:fk_j} using polynomial zonotope overapproximations of the joint position trajectories \eqref{eq:pz_pos}.
Using $\pzqji$ we can compute $\pz{p\jssmu}(\pzqji)$ and $\pz{R\jssmu}(\pzqji)$, which represent overapproximations of the position and orientation of the $j$\ts{th} frame with respect to frame $(j-1)$ at the $i$\ts{th} time step.

The rotation matrix $R\jssmu(q_j(t;k))$ depends on $\cos{(q_j(t;k))}$ and $\sin{(q_j(t;k))}$.
Because we represent a set of the $j$\ts{th} joint's angles for the $i$\ts{th} time step using the polynomial zonotope $\pzqji$, we must compute $\cos(\pzqji)$ and $\sin(\pzqji)$ to compute $\pz{R\jssmu}(\pzqji)$.
Cosine and sine are analytic functions, and so we can compute  $\cos{(\pzqji)}$ and  $\sin{(\pzqji)}$ using Taylor expansions as in  \eqref{eq:pz_taylor_inf}.
In practice, only a finite degree Taylor expansion can be constructed and the Lagrange Remainder as described in Sec. \ref{subsec:polyzono} is used to conservatively bound the truncation error. 
By using this property and the fact that all operations involving polynomial zonotopes are either exact or overapproximative, the polynomial zonotope forward kinematics can be computed similarly to the classical formulation \eqref{eq:fk_j} and proven to be overapproximative:
\begin{lem}[PZ Forward Kinematics]
\label{lem:PZFK}
Let the polynomial zonotope forward kinematics for the $j$\ts{th} frame at the $i$\ts{th} time step be defined as
\begin{equation}\label{eq:pzfk_j}
    \pzFKjKi = 
    \begin{bmatrix} \pz{R_j}(\pzqi) & \pz{p_j}(\pzqi)\\
    \mathbf{0}  & 1 \\
    \end{bmatrix},
\end{equation}
where
\begin{equation}
    \pz{R_j}(\pzqi) = \prod_{l=1}^{j} \pz{R_{l}^{l-1}}(\pzqli)
\end{equation}
and
\begin{equation}
    \pz{p_j}(\pzqi) = \sum_{l=1}^{j} \pz{R_l}(\pzqi) \pz{p_{l}^{l-1}},
\end{equation}
then for each  $j \in \Nq$,  $k \in \pz{K}$,  $\FK_j(q(t;k)) \in  \pzFKjki$ for all $t \in \pz{T_i}$.
\end{lem}
\noindent The Polynomial Zonotope Forward Kinematics Algorithm (PZFK), detailed in Alg. \ref{alg:compose_fk}, is used to compute the objects in Lem. \ref{lem:PZFK} from the set of possible configurations $\pzqi$.
\input{algorithms/pzfk}

\subsubsection{Forward Occupancy Reachable Set}
To guarantee safety, it is necessary to ensure that the robot never collides with any obstacles for all time.
To accomplish this, we overapproximate the forward occupancy \eqref{eq:forward_occupancy_j} of each link over every time interval.
By applying the forward kinematics reachable set \eqref{eq:pzfk_j} and the fact that all operations involving polynomial zonotopes are either exact or overapproximative, the polynomial zonotope forward occupancy reachable set can be computed and proven to be overapproximative: 
\begin{lem}[PZ Forward Occupancy]
Let the $j$\ts{th} link of the robot be overapproximated by a polynomial zonotope denoted by $\pz{L_j}$ and the polynomial zonotope forward occupancy reachable set for the $j$\ts{th} link at the $i$\ts{th} time step be defined as:
\begin{align}\label{eq:pz_forward_occupancy_j}
     \pzFOjKi = \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi)\pz{L_j},
\end{align}
then for each $j \in \Nq$,  $k \in \pz{K}$, $\FO_j(q(t;k)) \in  \pzFOjki$ for all $t \in \pz{T_i}$.
\end{lem}
\noindent In Sec. \ref{subsec:constraint_generation}, we describe how the forward occupancy reachable set is used to compute collision-avoidance constraints.
For convenience, let
\begin{equation}
    \label{eq:pz_forward_occupancy}
    \pz{FO}(\pzqi) = \bigcup_{j = 1}^{\nq} \pzFOjKi.
\end{equation}
\input{algorithms/pzfo}
%\input{algorithms/pzfk}





%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ REAL MAN STARTS HERE
% \begin{align}
%     \pz{R_j^{j-1}} = \{r\in \R^{3\times3} \, \mid \, r=C_r+\sum_{i=1}^{\pzn}G_{i,r}\,x^{\alpha}\}
% \end{align}
% where 
% \begin{align}
% C_r = I_{3\times3}+c_{\text{s}_{q,j}(T;K)}\,[w]_{\times}+(1-c_{\text{c}_{q,j}(T;K)})\,[w]_{\times}^2
% \end{align}
% and 
% \begin{align}
% G_{i,r} = g_{i,\text{s}_{q,j}(T;K)}\,[w]_{\times}-g_{i,\text{c}_{q,j}(T;K)}\,[w]_{\times}^2
% \end{align}
% with $[w]_{\times}$, a cross product matrix of joint axis vector, $w\in\R^3,\,|w|=1$. \yong{need to define PZ, indeterminant and exponent}
% \begin{itemize} 
%     \item FK based on transformation
%     \item FO from FK and link volume
% \end{itemize}

==> sections/reconstruction.tex <==
\section{RDF Approximation and Reconstruction}
In this section we describe how we overapproximate the distance between the Forward Occupancy reachable set and obstacles. We will also describe how the neural network architecture and how we generate the dataset



\begin{align}
    &\rdf_j(O, \pzk{\FO_j}) = \underset{p}{min} &&||p-c_{O}|| \\
    &&& p \in \conv(\bigcup_{i = 1}^{\nt}\pzki{\FO_{j,buf}}) 
\end{align}
where $\pzki{\FO_{j,buf}} = \pzki{\FO_j}\oplus Z_O^g$

==> sections/symbols.tex <==
\subsection{List of Symbols}

\begin{itemize}
%   \item $\int$:
%   \item $\pzg$
%   \item $\pzv$
%   \item $\pze$
%   \item $\pzn$
%   \item $\pzgi$
%   \item $\pzei$
%   \item $\interval{2}$:
%   \item $\pz{\dot{q}}$
%   \item $a_i$: DH parameter (link length?)
  \item $a_i^i$: acceleration of frame in expressed in frame i
  \item $a_{c,i}^i$: acceleration of link i com wrt frame i
  \item $a_0$: coefficient (but really center)
  \item $\pzei$: poly zonotope exponents
  % \item $\robgain$: robust input "gain"
%   \item $\alpha_i$: link twist in DH convention
  \item $\beta_i$: zonotope indeterminants
  \item $\beta_{\forall}$: all indeterminants of a zonotope
  \item $c$: zonotope center
  \item $\co$: obstacle center
%   \item $c$: shorthand for cosine
%   \item $c_i^i$: 
  % \item $c_{x_j}$: x-coordinate of COM of j-th link (same for y and z)
  % \item $C$: Matrix zonotope center
  % \item $C(q, \Delta)$: Coriolis matrix
%   \item $d_i$: DH parameter
  % \item $\Delta$: vector of inertial parameters
  % \item $\Delta_0$: vector of nominal inertial parameters
  % \item $[\Delta]$: vector of interval inertial parameters
  % \item $\pz{\Delta}$: vector of PZ inertial parameters
  \item $\dist(\cdot)$: distance function
  \item $\delta$: buffer threshold of \RDF collision-avoidance constraint 
  % \item $e$: vector of joint position errors
  % \item $\dot{e}$: vector of joint velocity errors
  % \item $\pbound$: ultimate position bound for single joint
  % \item $\vbound$: ultiamte velocity bound for single joint
  % \item $\pboundvec$: vector of ultimate position bounds
  % \item $\vboundvec$: vector of ultimate velocity bounds
  % \item $f_i^i$: Force at joint
  % \item $F_i^i$: Force at center of mass
  \item $\FK_i(q)$: forward kinematics
  \item $\FO_i(q)$: forward occupancy
  \item $\robcoeff$: robust input coefficient
  \item $g_i$: ith zonotope generator
  \item $g_{\forall}$: all generators of a zonotope
  \item $\pzgi$: ith PZ coefficient (aka generator)
  \item $G_i$:  ith generator matrix of Matrix zonotope 
  \item $G(q, \Delta)$: gravity vector
  \item $\kscale$: scale for $k$ interval
  % \item $\robh$: control barrier function
  \item $\robH$: forward invariant set associated with $\robh$
  \item $\Hjh=(\Ajh,\bjh)$: $h$-th half-space composing $\Pj$
  \item $i$: time index
  % \item $I_i^i$: link i inertia tensor wrt frame i
  \item $j$: joint index
%   \item $\mathcal{J}_i$: joint reachable set
%   \item $J_i(t)$: offline overapproximation of joint reachable set
  \item $k$: trajectory parameter
  \item $K$: space of trajectory parameters
  \item $K_r$: gain matrix
  % \item $\kappa_P$: robust controller gain
  \item $L_i$: volume of link i
%   \item $\lambda_j$: indeterminants
  % \item $\lambda_{min}$: smallest eigenvalue
  % \item $\lambda_{max}$: largest eigenvalue
  % \item $m_i$: mass of link i
  \item $M$: matrix zonotope
%   \item$\Mit$: matrix zonotope as a function of time
  % \item $M$: Mass matrix
  % \item $\pz{M}$: poly zonotope Mass matrix
  % \item $\pz{M(\pz{\q})}$: pz mass matrix as a function of pz state.
  % \item $M(\q, \Delta)$ true mass matrix at $\q$
  \item $n$: generic constant

  \item $\nd$: dimension of the environment
  \item $\nq$: number of joints
  \item $\nt$: number of time steps
  \item $\nhj$: number of halfspaces of $\Pj$
%   \item $n_{n_q}^{n_q}$: moment
  \item $\nObs$: number of obstacles
  \item $j\in\Nq$: $j\in\{1,\cdots,\nq\}$
  \item $i\in\Nt$: $i\in\{1,\cdots,\nt\}$
  \item $h\in\Nhj$: $h\in\{1,\cdots,\nhj\}$
  \item $\ell\in\NObs$: $\ell\in\{1,\cdots,\nObs\}$
  \item $N_i^i$: moment
  \item $O_j$: Obstacle $j$ where $j$ is a generic index
%   \item $\mathcal{O}$: set of all obstacles
  \item $\obsset$: set of all obstacles
  \item $\mathbb{N}$: natural numbers
  \item $\pzn$: number of PZ generators
  \item $p_1$: generic point inside poly zonotope
  \item $p_2$: generic point inside poly zonotope
  \item $p_i$: position of frame $i$ relative to frame $0$
  \item $p_{i-1,i}^i$: position of frame i wrt frame i-1 expressed in frame i \jon{i think this is not needed}
%   \item $PZ$: generic polynomial zonotope
  \item $\pz{P_1}$: generic polynomial zonotope
  \item $\pz{P_2}$: generic polynomial zonotope
  \item $\Pj$: convexhull of $j$-th link's buffered FRS
%   \item $\mathcal{ABCPZ}$: Polynomial Zonotope
%   \item $[\Phi]$: interval disturbance
%   \item $\varphi_P$: robust controller gain
  \item $q$: vector of joint positions
  \item $\qd$: vector of joint velocities
  \item $\qdd$: vector of joint accelerations
  \item $\initq$: estimate of initial position
  \item $\initdq$: estimate of initial velocity
  \item $\qdes$: desired joint positions
  \item $\qdesdot$: desired joint velocities
  \item $\qdesddot$: desired joint accelerations
  % \item $\qadot$: modified velocity trajectory
  % \item $\qaddot$: modified acceleration trajectory
  \item $\pzqji$: poly zonotope representation of $q$ at $i$\ts{th} time step
  \item $\pzqdji$: poly zonotope representation of $\qd$ at $i$\ts{th} time step
  \item $Q$: configuration space
  \item $\robr$: modified error
  \item $R_{i-1}^i$: orientation of frame $i-1$ \textit{wrt} frame $i$
%   \item $^{i}R_{i-1}$: orientation of frame $i-1$ \textit{wrt} frame $i$
  \item $R_i(q)$: orientation of frame $i$ \textit{wrt} frame $0$
  \item $\pz{R_{i-1}^i}$: poly zonotope representation of orientation of frame $i-1$ \textit{wrt} frame i
  \item $\mathbb{R}^n$: reals 
  \item $RDF$: Reachability-aware distance function
  \item $\rdf(\cdot)$: reachability-aware distance function
  \item $\ardf(\cdot)$: Analytical approximate of reachability-aware distance function
  \item $\rdfnn(\cdot)$: neural approximate of reachability-aware distance function
%   \item $\rho$: worst-case disturbance
%   \item $s$: shorthand for sine
%   \item $S_i(t)$: sliced reachable set
  \item $\sigma$: coefficient to be sliced/evaluated
  % \item $\sigma_m$: uniform bound
  % \item $\sigma_M$: uniform bound
  \item $t$: time
  \item $T$: time interval
  % \item $\tau$: nominal control input
  % \item $u$: control input
%   \item $U_i(t)$: overapproximation of input reachable set
  % \item $\robv$: robust control input
  % \item $\roblyap$: Lyapunov function
  % \item $\roblevel$: Lyapunov function threshold
%   \item $V_i(t)$: zonotope representation of link i volume
  \item $w$: disturbance due to inertial uncertainty
  \item $\normwmax$ norm of max disturbance
  \item $W$: workspace
  \item $\omega_i^i$: frame i angular velocity wrt frame i
  \item $\dot{\omega}_i^i$: frame i angular acceleration wrt frame i
  \item $\pzv$: indeterminant for polynomial zonotope
  \item $X$: a general set and/or metric space
  \item $\mathcal{X}$: set of input features
  \item $\mathcal{Y}$: set of labels
%   \item $x$: generic interval
%   \item $y$: generic interval
%   \item $z$: generic point inside zonotope
  \item $z_i$: frame i axis of rotation (expressed in base frame?)
  \item $Z$: generic zonotope
  \item $Z_1$: generic zonotope
  \item $Z_2$: generic zonotope
  \item $Z_1^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_1$
  \item $Z_2^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_2$

  %%% TRAINING and NETWORK SECTION
  \item $x$: input in dataset, input to network
  \item $y = (\Tilde{r}_1, \Tilde{r}_2)$: label in dataset
  \item $\hat{y} = (\hat{r}_1, \hat{r}_2)$: output vector from network
  \item $X$: input set in dataset
  \item $Y$: label set in dataset
  \item $\hat{Y}$: output set of network
  
\end{itemize}

\newpage
